Automatic Rumor Detection on Microblogs: A Survey

The ever-increasing amount of multimedia content on modern social media platforms are valuable in many applications. While the openness and convenience features of social media also foster many rumors online. Without verification, these rumors would reach thousands of users immediately and cause serious damages. Many efforts have been taken to defeat online rumors automatically by mining the rich content provided on the open network with machine learning techniques. Most rumor detection methods can be categorized in three paradigms: the hand-crafted features based classification approaches, the propagation-based approaches and the neural networks approaches. In this survey, we introduce a formal definition of rumor in comparison with other definitions used in literatures. We summary the studies of automatic rumor detection so far and present details in three paradigms of rumor detection. We also give an introduction on existing datasets for rumor detection which would benefit following researches in this area. We give our suggestions for future rumors detection on microblogs as a conclusion.

==> classification.tex <==
The basic definition of rumor detection is a binary classification problem. Most literatures on this task follows the commonly used learning paradigms of supervised classification from the study machine learning area: 1) extracting features representing samples from both classes; 2) training an appropriate classifier with provided samples; 3) testing and evaluating on unseen data. The first key step of these procedures is how to extract prominent features. On the other hand, contents are not independent and from different modalities. The classification method should be capable of integrating and interpreting these features for robust rumor detection. In this section, we first give a review of all kinds of features used in the rumor detection literatures. We then introduce typical classification models applied in rumor detection literatures.

In the scope of social media, a news story $e=\{M,U\}$ contains rich multi-modal resources as its content and associated with certain social context during its spreading, as shown in Figure \ref{fig_example}. Generally, features come from two main aspects of a story: its content and its social context(Figure \ref{fig_features}).

\begin{figure}
\centering
\includegraphics[width=3.3in]{example.png}
\caption{An example message on Weibo with some of its key features and contents marked.}

\label{fig_example}
\end{figure}

\subsection{Content Features}

For a news story $e$, the message set $M$ describes all the key information of it, which has content from three aspects:
\begin{itemize}
  \item Textual content: a text describing the news event. They provide details of the event and may contain certain opinions or sentiments towards the story.
  \item Images/Videos: sometimes a message will provide visual material to support its story.
  \item Other content: the specific communication style of social media would provide other informative content, such as hashtag topics(\#), user references(@), links to outer sources, and emoj icons, \emph{etc}.
\end{itemize}

Various content features are extracted from above primitive content, which can be categorized into two main types: textual features and visual features.

\subsubsection{Textual Features}
Compared with non-rumors, rumor texts are fabricated to mislead the public. Aiming to arouse much attention and stimulate the public mood, rumor texts tend to have certain patterns in contrast to non-rumor ones. For example, after analyzing a large amount of tweet streams, Zhao \emph{et al.} \cite{zhao2015enquiring} discover two types of language patterns in rumors: the correction type and the enquiry type. Thus, it is possible to extract features from the textual content, which can characterize rumors.

From different levels granularity of the language structure, various textual features are extracted to represent a rumor from the aspects of words, sentences, messages, topics and events.

General textual features are derived from the linguistics of a text, which are widely used in many natural language understanding tasks. Three categories of general textual features are commonly used in rumor detection tasks: lexical features, syntactic features, and topic features.

\begin{figure}
\centering
\includegraphics[width=3.5in]{features.pdf}
\caption{Main categories of features used for rumor detection on microblogs.}

\label{fig_features}
\end{figure}

\textbf{Lexical features} are features extracted at the word-level of a rumor, which could be statistics of words, lexical rumor patterns or sentimental lexicons:

\begin{itemize}
  \item
  In \cite{castillo2011information}, the authors compute some statistics of rumor texts based on the words it contains, including the total number of words and characters, the number of distinctive words and the average length of word in a rumor, \emph{etc}. Apart from simple statistical features, some work extract interesting lexical words by examining their semantics.
  \item
  According to the study of \cite{zhao2015enquiring}, the informative part of rumor messages can be of the following two types: inquiries of the event situation (verification/confirmation questions) and corrections/disputes of the event. They detect the inquiry and correction patterns of rumor messages through supervised feature selection on a set of labeled messages. Specifically, the uni-grams, bi-grams, and tri-grams lexical parts are extracted from these messages after standard word segmentation. Frequency features (tf) of each extracted word or phrase are then calculated. Following that, Chi-Squared test and information gain ratio method are utilized to select prominent patterns. The feature selection methods rank features based on their ability to distinguish rumor tweets from non-rumor ones. From the ranked list of features, human experts select event-independent phrases as final lexical patterns for rumors. Finally, the lexical word patterns are discovered, including verification patterns ( ``is it real/fake?", ``need more evidence/confirmation", \emph{etc.}) and correction patterns ( ``rumor/false rumor", ``spreading/ fabricating rumor", \emph{etc.}). Once discovered these lexical features can be used to filter out rumors in real time, such as detect rumors in live tweet streams \cite{zhao2015enquiring}\cite{jinImage} or analyzing online rumors at a large scale\cite{jin2017Rumor}.
  \item
  Lexical words expressing specific semantics or sentiments are also very important clues to characterize the text. In \cite{castillo2011information}, the occurrence times of pronouns, emotional marks( question mark and exclamation mark) and emotion icons are counted as textual features. 
  
  %The occurrences of popular named entities of people, location and organization within a rumor event are unutilized as lexical features in [].%

  In \cite{kwon2013prominent}, many sentimental lexical features are proposed based on sentiment dictionary.   Specifically, they utilize a sentiment tool called the Linguistic Inquiry and Word Count (LIWC) to count words in psychologically meaningful categories. For each input text, this tool provides sentiment analysis results on five major categories and a number of subcategories, such as social, affective, cognitive, perceptual, and biological processes. After comparative study of these features, they find that some categories of sentiments are distinctive features for rumor detection, including positive affect words, cognitive action words and tentative action words.


\end{itemize}

\textbf{Syntactic features} represent rumors at the sentence level.

\begin{itemize}
  \item
  The basic syntactic features are simple statistics of a rumor message, such as the number of keywords, the sentiment score or polarity of the sentence\cite{castillo2011information} and part-of-speech tagging \cite{hassan2010s}.
  \item
  To represent a document based on the words it contains, the bag-of-words (BoW) language model is commonly utilized. In this model, each text document is represented as a $v$-dimensional vector, where $v$ is the size of the dictionary of the corpus. Each element in the vector stands for the TF-IDF score of the corresponding word in the text. TF is the term frequency. IDF score is the inverse document frequency, which is calculated on the whole corpus. Some work utilized BoW for rumor detection \cite{ma2017content} or rumor analysis \cite{jin2017Rumor}.
  \item
  Recently, semantic embedding algorithms are widely used in many natural language understanding applications. The Word2Vec model \cite{mikolov2013distributed} represents each word in a corpus with a real-valued vector in a common semantic vector space. This algorithm models words based on their semantic analogies. Inspired by its success, some recent rumor detection applications \cite{ma2017content}\cite{jin2017Rumor} also represent texts via word embedding.

\end{itemize}


\textbf{Topic features} are extracted from the level at the message set, which aim to understand messages and their underlying relations within a corpus.

Wu \emph{et al.} \cite{wu2015false} define a set of topic features to summaries semantics for detecting rumors on Weibo. They train a Latent Dirichlet Allocation (LDA) \cite{blei2003latent} model with an 18-topic distribution on all messages. And each message can belong to one or more topics. They transform the 18-dimensional distribution vector into binary vector by setting the top $k$-highest probability topics to 1 and the rest of topics to 0. The size of $k$ is selected based on the coverage of remained topics.

Jin \emph{et al.} \cite{jin2015} cluster topics based the event a message refers to and extract features both at the message level and the topic level. They assume that messages under a same topic probably have similar credibility values. Under this assumption, they cluster messages into different topics and obtain the topic-level feature by aggregating features on the message level. They claim that this kind of topic-level feature can reduces the impact of noisy data while maintaining most of details on the message level.

Towards a more comprehensive understanding of text on social media, existing work also come up with textual features derived from the traits of social media platform, apart from general textual features. For example, features extracted from outer source links \cite{zhang2015predictors}.


\subsubsection{Visual features}
While most work detects rumors depend on textual content, only some very recent work try to extract features from the visual content of rumors.

Gupta \emph{et al.} \cite{gupta2013faking} make a first attempt to understand the temporal, social reputation and influence patterns for the spreading of fake images on Twitter. They propose a classification model to identify the fake images on Twitter during Hurricane Sandy. Some interesting conclusions are drawn: the original fake images are limited, and 86\% of fake images were re-tweets. These findings could be utilized to design prominent visual features for rumor detection. However, their work is mainly based on traditional textual features.

Aiming to automatically predict whether a tweet that shares multimedia content is fake or real, Boididou \emph{et al.} \cite{verifying2015} proposed the Verifying Multimedia Use task that took place as part of the MediaEval benchmark in 2015 and 2016. This task attracts attentions for verifying images in tweets from the research area.

Visual features are features characterizing the visual content(images or videos) from different aspects. Regarding the methods of feature extraction, visual features can be categorized into three types: visual statistical features, visual content features, and visual embedding features.

\textbf{Visual statistical features} are statistics of images attached in rumors. Similar to the statistical features of textual content, some basic statistics of images proved to be distinctive in separating rumors and non-rumors. 

Gupta \emph{et al.} \cite{gupta2012evaluating} define a feature to record whether the user has a profile image for evaluating the credibility of user. A ``has multimedia" feature is defined in \cite{wu2015false} to record the status of multimedia attachment of a tweet: whether the tweet has any picture, video or audio attached. In \cite{sun2013detecting}, the authors point out that the rumors are more likely to contain outdated images. They propose a time span feature to capture this time delay. In \cite{zhang2015predictors}, the relation of images and health related rumors were studied. The Baidu search engine is deployed to find the original image for calculating this time span between the original image and the current one. According to their results, this feature is quite effective. However, the sparsity of outdated images and the difficulties to search them limit the usage of this feature.

Summarizing existing statistical features and proposing several novel features, seven visual statistical features are presented in \cite{jin2017Novel} from three aspects:

\begin{itemize}
  \item Count: Users can post zero, one or more than one images along with a text content in a tweet. To mark the occurrence of images in rumor messages, they count the total images in a rumor event and the ratio of messages containing at least one or more than one images.
  \item Popularity: Some images are very popular and gain more re-tweets and comments than others in an event. The ratio of the most popular images are calculated to denote this feature.
  \item Image type: Some images have particular type in resolution or style. For example, long images are images with a very large length-to-width ratio. The ratio of these types of images is also counted as a statistical feature.
\end{itemize}

\textbf{Visual content features} are extracted to describe image distributions from a visual perspective, such as visual clarity, diversity and coherence.


In \cite{jin2017Novel}, the authors find that images in rumors and non-rumors are visually distinctive on their distributions. To describe image distributions based on the visual content, five image visual features are proposed in their work: visual clarity score, visual coherence score, visual similarity distribution histogram, visual diversity score, and visual clustering score, which describe image distribution characteristics from different visual aspects.

\begin{itemize}
  \item
  \textbf{Visual Clarity Score} measures the distribution difference between two image sets: one is the image set in a certain news event (event set) and the other is the image set containing images from all events (collection set) \cite{hauff2008improved}. This feature is designed under the assumption that a non-rumor event would contain many original images specifically related to this event, which have a different image distribution in comparison with the overall image set.

  The clarity score is defined as the Kullback-Leibler divergence\cite{kullback1951information} between two language models representing the target image set and all image set, respectively. The bag-of-word image representation is employed to define language models for images. To be specific, local descriptors (e.g. the scale-invariant feature transform (SIFT)\cite{lowe2004distinctive} feature) for each image are extracted and then quantized to form a visual word vocabulary. Each image is represented by words from the vocabulary.

  \item
  \textbf{Visual Coherence Score}  measures how coherent images in a certain news event are \cite{he2008using}\cite{tian2012query}.
 This feature is computed based on visual similarity among images and can reflect relevant relations of images in news events quantitatively.
  More specifically, the average of similarity scores between every two images is computed as the coherence score. In implementation, the similarity between image pairs is calculated based on their GIST feature representations \cite{oliva2001modeling}.

  \item
  \textbf{Visual Similarity Distribution Histogram} describes inter-image similarity in a fine granularity level. It evaluates image distribution with a set of values by quantifying the similarity matrix of each image pair in an event\cite{tian2012query}.
  The visual similarity matrix is obtained by calculating pairwise image similarity in an event. The visual similarity is also computed based on their GIST feature representations. The image similarity matrix is then quantified into an $H$-bin histogram by mapping each element in the matrix into its corresponding bin, which results in a feature vector of $H$ dimensions representing the similarity relations among images.

  \item
  \textbf{Visual Diversity Score} measures the visual difference of the image distribution. Compared with visual coherence score, it computes the image diversity distribution directly and gives more emphasis on representative images.

  The diversity of an image is defined as its minimal difference with the images ranking before it in the whole image set\cite{wang2010}. Here images are ranked according to their popularity on social media, based on the assumption that popular images would have better representation for the news event. The visual diversity score is then calculated as a weighted average of dissimilarity over all images, where top-ranked images have larger weights \cite{deselaers2009jointly}. So that this feature can reduce the impact of unpopular noisy images. Dissimilarity of an image pair is computed as the complementary of its similarity.

  \item
  \textbf{Visual Clustering Score} evaluates the image distribution from a clustering perspective. It is defined as the number of clusters formed by all images in a news event.

  To cluster images, the hierarchical agglomerative clustering (HAC) algorithm \cite{king1967step} is employed, which merges nearest atomic clusters into larger clusters in a bottom-up strategy. HAC does not require the number of clusters to be determined or estimated before clustering. Thus, the number of clusters yielded by HAC reveals the diversity feature of images.

  In implementation, the single-link strategy is used to measure the similarity between two clusters, and the Euclidean distance of image GIST feature vectors is used as the distance measurement. Very small clusters are considered as outliers and removed before calculating the final score \cite{jin2017Novel}.
\end{itemize}

Evaluation of these visual content features on a set of 25,513 images from 146 events shows that images in rumors are more coherentm less diverse and  forming less clusters compared with those in non-rumors. Consequently, these feature can be useful for detecting rumor events.

\textbf{Visual embedding features} are learned through the state-of-the-art image embedding neural networks on a large dataset. It contains rich semantics of an image.

Recently, Convolutional Neural Networks (CNN) have shown a promising result on learning image representation and capturing semantic meaning of images. For many computer vision problems, including image classification \cite{krizhevsky2012imagenet} \cite{simonyan2014very} and object detection \cite{girshick2014rich} \cite{szegedy2013deep}, CNN have shown the superiority to traditional models based on hand-crafted features. Inspired its success in learning accurate image representation, some recent work seeks to it for understanding images in rumor detection task. In \cite{jin2017multimodal}, the authors utlize a VGG-net\cite{simonyan2014very} pre-trained with ImageNet dataset, a widely used CNN model in image understanding area, to extract features for images in rumor messages.

To directly learn the embedding of images in rumors, \cite{jinImage} propose an iterative transfer learning approach based on CNN.
As there are not sufficient labeled rumor images to learn such a robust deep neural networks, Jin \emph{et al.} resolve to the transfer learning paradigm in their approach. The proposed method has three main procedures:
\begin{enumerate}
  \item Constructing an auxiliary image set directly related to images in rumors. A large amount of automatically collected images are collected based on the text mining on the surrounding rumor texts of images. These images are have machine-generated weak labels and contains related knowledge for the target task of learning rumor images representation.
  \item Training a Convolutional Neural Network with both the auxiliary data and the target training data. To eliminate the effects of wrong labels in the auxiliary dataset, this CNN is designed to train with weighted instances, where each input image has different weight according to the training error.
  \item Iterative transfer learning. To overcome the distributional difference between two datasets and the label inaccuracy issue in the auxiliary set, an adaBoost-like algorithm is proposed to gradually adjusting the weight of each instance accordingly during model learning.
\end{enumerate}

\subsection{Social context features}
Social media is defined as an online multimedia platform for user engaging, community formation and social interaction. One of its key feature is its openness for all kinds of interactions, in comparison with traditional media.  Three types of social interactions universally exit on social media:

\begin{itemize}
  \item Interactions among users, such as ``adding friend" and ``following''. This kind of interaction forms the huge and complex underlying network where all information circulates.
  \item Links among multimedia content are formed through tags, hashtag topics or url links. Online contents are organized into sub-groups with this kind of links.
  \item Interactions among users and content, such as ``posting'',``commenting'', ``reposting'', and ``tagging''.
\end{itemize}

Many features are derived from the social connection characteristic of social media on the rumor detection task. Three main types of social features are user feature, propagation features and temporal features.

\textbf{User features} are derived from the user social network. Rumors are created by a few users and spread by many users. Analyzing their characteristics could provide crucial clues for rumor detection. User features could describe the characteristics of a single user or a user group comprised of multiple related users.

\begin{itemize}
  \item
  Individual features are extracted from single user. Common individual features are calculated from a user's  profile, such as ``register time'', ``age'', ``gender''and ``occupation'' \cite{morris2012tweeting}, or user's online actions, such as ``number of followers'', ``number of followees'' and ``number of posted messages'' \cite{castillo2011information}.

  Yang \emph{et al.} \cite{yang2012automatic} proposed two features to mark the user's posting behavior: the ``client'' feature is the software that was used by the user and the ``location'' feature marks whether the message is sent from from where the event happened or not.

  Liu \emph{et al.} \cite{liu2015real} evaluated a user's reliability from the perspective of journalists and proposed user features including the credibility identification, diversity and location of a source user.

  \item Group features are  overall features of a group whose members have certain similar behaviors in the rumor diffusion process \cite{yang2012automatic}. Group features can be generated by aggregating features of single user, such as ``the ratio of verified users'' and ``the average followee count''.
\end{itemize}

\textbf{Propagation features} are derived from the fusion network on which rumors spread. In \cite{castillo2011information}, some statistics of messages' propagation trees, such as the average depth or size of propagation trees, were proposed to capture basic propagation features. The work of Kwon \emph{et al.} \cite{kwon2013prominent} further extended them with 15 structural features extracted from the diffusion network as well as the user friendship network, including the number of nodes and links, the median degree and density of these networks. Wu \emph{et al.} \cite{wu2015false} proposed a concise structure to describe the propagation process for a single message. Yang \emph{et al.} \cite{yang2015exploiting} proposed a set of network features based on network created via the comment providers. In \cite{wang2015detecting}, certain propagation structures are studied to find the distinctive patterns for rumor detection.

\textbf{Temporal features} mark the import time points or the life circle pattern about the diffusion of rumors. In  \cite{kwon2013prominent} message spikes along the time line are modeled to capture the spreading patterns of rumors. Ma \emph{et al.} \cite{ma2015detect} proposed a method for discretizing time stream and capturing the variation of time features. Giasemidis \emph{et al.} \cite{giasemidis2016determining} split every rumor events into 20 time-intervals and extract features for each subset of messages.

Kwon \emph{et al.} studied the stability of features over time \cite{kwon2017rumor}. They found that for rumor detection linguistic and user features are suitable for early stage, while structural and temporal features tend to have good performance in the long-term stage.

\subsection{Classification Methods}
With sufficient features available, many classification methods are proposed in literatures focusing on finding effective features for the rumor detection task.

Most work experimented with more than one classifiers to find the most suitable method, including Decision Tree \cite{castillo2011information}\cite{ma2015detect}\cite{giasemidis2016determining}, Bayesian networks\cite{castillo2011information}, Random Forest\cite{kwon2013prominent}\cite{jin2017Novel}, Logistic Regression \cite{giasemidis2016determining}\cite{zhang2015predictors} and SVM\cite{castillo2011information}\cite{kwon2013prominent}\cite{yang2012automatic}\cite{jin2017Novel}\cite{ma2015detect}.


Some work proposed novel classification algorithms for better aggregating diverse features.  Wu \emph{et al.} \cite{wu2015false}
proposed an SVM with a hybrid kernel technique consisting of random walk kernel \cite{borgwardt2005protein} and an RBF kernel \cite{buhmann2003radial}. The random walk kernel is specifically designed to capture propagation features from the comments tree of a message, while the RBF kernel is applied on content and user features. A two-level classification framework was proposed in \cite{jin2015} to leverage features at the message-level and topic-level. Regarding rumors as anomalies, Chen \emph{et al.}  \cite{chen2016behavior} initially used anomaly detection to classify rumors. 

